Compositional Image Retrieval via Instruction-Aware Contrastive Learning

Composed Image Retrieval (CIR) involves retrieving a target image based on a composed query of an image paired with text that specifies modifications or changes to the visual reference. CIR is inherently an instruction-following task, as the model needs to interpret and apply modifications to the image. In practice, due to the scarcity of annotated data in downstream tasks, Zero-Shot CIR (ZS-CIR) is desirable. While existing ZS-CIR models based on CLIP have shown promising results, their capability in interpreting and following modification instructions remains limited. Some research attempts to address this by incorporating Large Language Models (LLMs). However, these approaches still face challenges in effectively integrating multimodal information and instruction understanding. To tackle above challenges, we propose a novel embedding method utilizing an instruction-tuned Multimodal LLM (MLLM) to generate composed representation, which significantly enhance the instruction following capability for a comprehensive integration between images and instructions. Nevertheless, directly applying MLLMs introduces a new challenge since MLLMs are primarily designed for text generation rather than embedding extraction as required in CIR. To address this, we introduce a two-stage training strategy to efficiently learn a joint multimodal embedding space and further refining the ability to follow modification instructions by tuning the model in a triplet dataset similar to the CIR format. Extensive experiments on four public datasets: FashionIQ, CIRR, GeneCIS, and CIRCO demonstrates the superior performance of our model, outperforming state-of-the-art baselines by a significant margin. Codes are available at the GitHub repository.

==> suppl_ex.tex <==
\clearpage
\setcounter{page}{1}

\maketitlesupplementary
\renewcommand{\thesection}{\Alph{section}}
\setcounter{section}{0}

\section{Related Works}
\subsection{Instruction Tuning}
Instruction tuning~\citep{zhang2023instruction, ouyang2022training, chung2024scaling, zheng2023judging} is a strategy commonly adopted in modern LLM training to enhance model generalization by exposing models to various prompts. In the realm of multimodal large language models (MLLMs), visual instruction tuning~\citep{liu2024visual} has significantly improved their instruction-following capabilities when processing multimodal data. This process typically involves two stages: the first stage trains an adapter between the visual encoder and the LLM using image captioning data; in the second stage, the LLM and the adapter are jointly trained with instruction-following data that encompasses multiple tasks in a question-answer format. While previous MLLMs have primarily focused on text generation, recent research is exploring the use of LLMs for representation learning. Specifically, E5-Mistral~\citep{wang2023improving} leverages LLMs as embedding models by training them on various retrieval tasks specified by instructions. E5-V~\citep{jiang2024e5} extends this approach to multimodal domains; however, its training remains based on pure text pairs, and the full potential of MLLMs for multimodal embeddings is not fully realized. In this paper, we propose a novel approach to train an instruction-aware model that generates multimodal embeddings through two stages: embedding alignment and instruction contrastive learning.

\subsection{Composed Image Retrieval}
% Composed Image Retrieval (CIR) refers to finding related images from a source image under a condition, usually a modifier text. Such a task finds real-world applications in e-commerce, recommendation, etc. Due to the difficulty of acquiring specific datasets to different CIR tasks, recent research is exploring the Zero-Shot CIR (ZS-CIR). Previous methods mostly explore representing the reference image to specific tokens and concatenating them with text tokens for retrieval~\cite{saito2023pic2word, karthik2023vision, tang2024context, suo2024knowledge, agnolucci2024isearle,gulanguage}. With the advents of Multimodal Large Language Models (MLLMs), some researchers seek to incorporate LLMs in this domain. CIReVL~\cite{karthik2023vision} leverages two MLLMs, one for generating image captions and the other for combining captions and modifier texts for retrieval. FROMAGe~\cite{koh2023grounding} and MCL~\cite{liimproving} explore using LLMs for embeddings. But the LLMs are mainly used as the text encoder. Thanks to the rapid development of MLLMs, modern MLLMs exhibit strong generalization, instruction-following, and zero-shot capability in multimodal data. However, their applications on CIR tasks is rarely explored. In this paper, we leverage MLLMs as embedding models for CIR tasks, where the image and modifier text can be directly encoded by a single model.
Composed Image Retrieval (CIR) involves finding images related to a source image under a specified condition, typically provided as a modifier text. This task has practical applications in e-commerce, recommendation systems, and more. Due to the difficulty of acquiring specific datasets for various CIR tasks, recent research has focused on Zero-Shot CIR (ZS-CIR). Previous methods primarily represent the reference image as specific tokens and concatenate them with text tokens for retrieval~\citep{saito2023pic2word, karthik2023vision, tang2024context, suo2024knowledge, agnolucci2024isearle,gulanguage}. With the advent of Multimodal Large Language Models (MLLMs), researchers have begun incorporating LLMs into this domain. For instance, CIReVL~\citep{karthik2023vision} leverages two MLLMs: one for generating image captions and another for combining captions with modifier texts for retrieval. FROMAGe~\citep{koh2023grounding} and MCL~\citep{liimproving} explore using LLMs for embeddings, but the LLMs are mainly used as text encoders. Despite the rapid development of MLLMs exhibiting strong generalization, instruction-following, and zero-shot capabilities in multimodal data, their applications to CIR tasks are rarely explored. In this paper, we leverage MLLMs as embedding models for CIR tasks, enabling direct encoding of images and modifier texts within a single model.
\begin{figure*}[!h]
    \centering
    \includegraphics[width=0.9\linewidth]{images/data_generation.pdf}
    \caption{We prompt GPT-4o to generate triplet data from CC3M. Our prompt consists of three parts: the first part (\textcolor{orange}{orange}) defines the task we aim to complete; the second part (\textcolor{myblue}{blue} and \textcolor{mypurple}{purple}) specifies the details and requirements of the task; and the third part (\textcolor{black}{black}) provides examples for triplet generation, where the modifier text is brainstormed step by step. The key concepts in the captioned are identified and subsequently selected concepts are altered. The modified caption is derived accordingly. Finally, we provide the input (\textcolor{red}{red}). GPT then outputs the modifier text and the corresponding caption based on the query caption (\textcolor{mygreen}{green}).}
    \label{fig: gpt_prompt}
\end{figure*}

\section{Dataset Details}
\label{sec: data_detail}
We evaluate our model using four well-established zero-shot CIR benchmarks: FashionIQ~\citep{guo2019fashion}, CIRR~\citep{Liu_2021_ICCV}, CIRCO~\citep{baldrati2023zeroshot}, and GeneCIS~\citep{vaze2023genecis}. While FashionIQ is an early benchmark for CIR, its domain is restricted to fashion e-commerce images. In contrast, CIRR and CIRCO focus on more general natural images. CIRR is the first CIR dataset centered on natural images, but it suffers from the limitation of having only one target image per query, leading to potential false negatives. On the other hand, CIRCO improves upon this by providing multiple target images per query, which reduces the likelihood of false negatives and offers a more comprehensive evaluation of retrieval accuracy. 
GeneCIS is a dataset for conditional image retrieval. It defines four types of conditions as focusing or changing attributes or objects in images. In line with common practice, we report Recall@k ($R@k$) for FashionIQ, CIRR, and GeneCIS, with an additional subset metric for CIRR denoted as $R_s@k$. For CIRCO, where multiple correct images can correspond to a single query, we use mean Average Precision ($mAP@k$) to capture both precision and recall across different retrieval positions. 

\section{Triplet Data Generation}
\label{sec: triplet_data}

\subsection{Data Processing}
We utilize GPT-4o~\citep{achiam2023gpt} to process and generate triplet data. Given an image and its caption, we use the caption as a prompt to GPT, which then derives the modifier text and the modified caption. The detailed prompt structure is shown in Figure \ref{fig: gpt_prompt}. Specifically, the prompt is divided into three parts: task definition, requirements, and few-shot examples.

Our data generation process differs from MCL~\citep{liimproving} in several aspects. First, we leverage GPT-4o~\citep{achiam2023gpt} instead of LLAMA2~\citep{touvron2023llama}, allowing for more generalizable and creative content generation. Second, GPT-4o has a larger context window, enabling us to incorporate more complex techniques within the prompt. Unlike MCL, which directly presents the output modifier text and corresponding caption in few-shot examples, we divide the generation process into several steps using the Chain of Thought method~\citep{wei2022chain}. We instruct GPT to first identify key points in the example caption, then selectively alter some of them as modifications, and finally derive the modified caption. This step-by-step generation ensures that the generated modifier text and corresponding caption are reasonable and closely related to the original caption. \textit{At the time the major work of this paper is finished, the MCL dataset has not been released. We will defer the comparison between two datasets in the future work.}

Our pipeline differs from the training set derivation in \citep{vaze2023genecis}. While they use text scene graphs to identify subjects, predicates, and objects, their modifier instruction is generated by simply replacing one element with another concept from the dataset, leading to limited creativity and diversity.

\begin{table}
\centering
\begin{tabular}{c|c}
\hline
\textbf{Dataset} & \textbf{Approx. Size} \\ \hline
FOIL~\cite{shekhar2017foil_acl} & 60K  \\
LLaVA-Pretrain~\cite{liu2024visual} & 558K \\
CC3M-Instruct & 300K \\
\hline
\end{tabular}
\caption{Approximate Sizes of Different Datasets}
\label{tab: dataset_size}
\end{table}

\begin{table*}[!h]
\centering
\scalebox{0.9}{
\begin{tabular}{l|p{11cm}}
\hline
Task & Instruction Template \\
\hline
\multirow{13}{*}{\shortstack{Image \\ Modification}} & \texttt{<Image>} The image is conditioned on the following prompt: \{modifier text\}, summarize the image and the prompt to retrieve a description of the image changed by the condition: \\
                                   & \texttt{<Image>} Given the image conditioned by the prompt: \{modifier text\}, condense the essence of the image and the prompt into a single word to fetch a description of the altered image: \\
                                   & \texttt{<Image>} Using the prompt to condition the image: \{modifier text\}, provide one word that encapsulates the overall concept of the conditioned image to retrieve its description: \\
                                   & \texttt{<Image>} Based on the image influenced by this prompt: \{modifier text\}, distill the description of the conditioned image and the prompt into one word to access the altered description: \\
                                   & \texttt{<Image>} With the image modified according to the prompt: \{modifier text\}, summarize both the image and the prompt to obtain a description of the conditioned image: \\
                                   & \texttt{<Image>} Condition the image with this condition: \{modifier text\}. Summarize the result: \\
                                   & \texttt{<Image>} Using this prompt: \{modifier text\}, describe the conditioned image: \\
                                   & \texttt{<Image>} Apply the prompt: \{modifier text\} to the image. Provide one word for the conditioned image: \\
                                   & \texttt{<Image>} Given this prompt: \{modifier text\}, condense the conditioned image into one word: \\
                                   & \texttt{<Image>} \{modifier text\}: \\ \hline
% \multirow{10}{*}{\shortstack{Image \\ Summary}} & \texttt{<Image>} Summary: \\
%                       & \texttt{<Image>} Caption: \\
%                       & \texttt{<Image>} Summarize the image for retrieval: \\
%                       & \texttt{<Image>} A short image caption: \\
%                       & \texttt{<Image>} A short image description: \\
%                       & \texttt{<Image>} Provide a description of what is presented in the photo: \\
%                       & \texttt{<Image>} Please provide a short depiction of the picture: \\
%                       & \texttt{<Image>} Using language, provide a short account of the image: \\
%                       & \texttt{<Image>} Use a word to illustrate what is happening in the picture: \\ \hline
\multirow{6}{*}{\shortstack{Caption \\ Summary}} & \texttt{<Caption>} Summary: \\
                     & \texttt{<Caption>} Summarize the caption for retrieval: \\
                     & \texttt{<Caption>} A shorter description is: \\
                     & \texttt{<Caption>} Shorter caption: \\
                     & \texttt{<Caption>} “”\\ \hline
\end{tabular}
}
\caption{Instruction templates for different tasks. In \textbf{Image Modification}, the modifier text combined with the selected template serves as the formatted prompt. \textbf{Caption} \textbf{Summary} instruct the model to generate a global representation for captions.}
\label{tab: prompt_template}
\end{table*}

\subsection{Data Details}
\label{sec: data_stats}
After filtering invalid images and failed prompts, we acquire the CC3M-Instruct dataset with 2M triplets. We randomly sample 300K triplets to maintain the training efficiency as well as performance. Triplet examples are shown in Figure \ref{fig: vis_example}. In our experiments, the first stage of training takes about 1.5 hours while the second stage of training takes about 2.5 hours. Table \ref{tab: dataset_size} shows the sizes of training datasets. Note that in the second training stage, we use in-batch samples as negatives as well as the original caption of the current triplet as the hard negative.

\section{Prompt Templates}
\label{sec: prompt_tempalate}
Templates for training are shown in Table \ref{tab: prompt_template}.

\subsection{Templates for Training}
In our second training stage, we use two prompt templates for the source image and modification instruction, and the target caption. Both templates are sampled from predefined template sets, respectively. Table \ref{tab: prompt_template} shows both template sets we used.

\subsection{Templates for Zero-shot Inference}
We use different prompt template for inference. In inference, the source image and modification instruction are formatted in a prompt. The target image are composed with a summary prompt. Both are encoded by InstructCIR and a consine similarity is computed between their embeddings.

\textbf{CIRR \& CIRCO}

\textit{Image Captioning}

\texttt{<Image>} Describe this image in one word: 

\textit{Image Modification}

\texttt{<Image>} Modify this image with \{modifier text\}, describe the modified image in one word: 

\textbf{FashionIQ}

\textit{Image Captioning}

\texttt{<Image>} Describe this \{data type in fashioniq\} in one word based on its style: 

\textit{Image Modification}

\texttt{<Image>} Modify the style of this \{data type in fashioniq\} based on \{modifier text\}. describe this modified \{data type in fashioniq\} in one word based on its style: 

\textbf{GeneCIS}

\textit{Image Captioning}

\texttt{<Image>} Summarize the image for retrieval: 

\textit{Image Modification}

\texttt{<Image>} Describe the image in one word with a specific focus on the attribute \{specific attribute\}:

\texttt{<Image>} Describe the image in one word with a specific change of the attribute \{specific attribute\}:

\texttt{<Image>} Describe the image in one word with a specific focus on the object \{specific object\}:

\texttt{<Image>} Describe the image in one word with a specific change of the object \{specific object\}:

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{images/attention_map_example.pdf}
    \caption{\textbf{Qualitative Examples of Attention Maps.} Before training, the model can only or cannot focus on specific objects in the image according to the instruction. After the training, the model is able to capture these objects. In the example above, the model highlights the front wheel and floor. In the example below, the model high lights the main side of the bus.}
    \label{fig: attn_exam}
\end{figure}

\section{Attention Map Analysis}
\label{sec: attn_map_analy}
In this section, we analyze what InstructCIR learns for composed image retrieval. Specifically, we aim to investigate which parts of the original image contribute the most to the composed embedding. Note that the composed embedding contains both the image and instruction. Therefore, the most significant parts are supposed to be indicated by the instruction instead of just the major ones. Inspired by \cite{yu2024attention} that creates attention maps highlighting instruction-aware image patches, we conduct qualitative analysis through attention maps. Specifically, InstructCIR leverages the [EOS] token embedding from the output sequence as the composed embedding $h_{it}$. Similar to \cite{yu2024attention}, we compute the similarity between the composed embedding $h_{it}$ and patch embeddings $H=\{h_1, h_2,\cdots,h_{P^2}\}$ in the output sequence, where $P$ is the number of image patches. The patch similarity is resized to the grid shape $S \in \mathbb{R}^{P\times P}$. The similarity grid is finally interpolated to the attention map $A \in \mathbb{R}^{H\times W}$, where $H$ and $W$ are the height and width of the image. 

\begin{equation}
\begin{aligned}
    S &= H \cdot (h_{it})^T, S\in \mathbb{R}^{P^2} \\
    S &= \text{Resize}(S), S\in \mathbb{R}^{P\times P} \\
    A &= \text{Interpolate}(S), A \in \mathbb{R}^{H\times W}
\end{aligned}
\label{equ: attn_cal}
\end{equation}

The attention map is mixed with the image in the alpha channel, highlighting important objects in the image. Examples are shown in the Figure \ref{fig: attn_exam}, demonstrating the original image, attention maps before and after training the model. 
Before training, the original model (LLaVA-Phi) focuses on the main object in the image. In the first example, it mainly focuses on the motorman. After training, the model is able to pay higher attention on specific parts mentioned in the image, i.e., the front wheel and the floor, than other parts. The qualitative analysis highlights the instruction-awareness of the model trained with the two-stage strategy. 

\begin{table}[ht]
\centering
\begin{tabular}{c|c}
\hline
\textbf{Config} & \textbf{Value} \\ \hline
Visual Encoder & openai/clip-vit-large-patch14 \\
Image Resolution & 224x224 \\
Language Model & microsoft/Phi-3.5-mini-instruct \\
Adapter & MLP \\
Pretraining Strategy & Frozen LLM, Frozen ViT \\
Fine-tuning Strategy & Full LLM, Full ViT \\
Pretrain Dataset & ShareGPT4V-PT (1246K)~\citep{chen2023sharegpt4v} \\
Fine-tune Dataset & InternVL-SFT (1268K)~\citep{chen2024internvl} \\
Pretrain Epoch & 1 \\
Fine-tune Epoch & 2 \\
\hline
\end{tabular}
\caption{Configurations of Training LLaVA-Phi}
\label{tab: mllm_config}
\end{table}

\begin{table}[ht]
\centering
\begin{tabular}{c|c}
\hline
\textbf{Model} & \textbf{Size} \\ \hline
xtuner/llava-phi-3-mini-hf & 4.14B  \\
microsoft/Phi-3.5-vision-instruct & 4.15B \\
E5-V & 8.35B \\
\hline
\end{tabular}
\caption{Number of parameters of different models}
\label{tab: model_size}
\end{table}

\begin{table*}[!ht]
\centering
\scriptsize
% \setlength{\tabcolsep}{5pt}
\begin{tabular}{cccccccccccccc}\toprule
\multirow{2}{*}{\multirow{2}{*}{Method}} &\multicolumn{3}{c}{\textbf{Focus Attribute}} &\multicolumn{3}{c}{\textbf{Change Attribute}} &\multicolumn{3}{c}{\textbf{Focus Object}} &\multicolumn{3}{c}{\textbf{Change Object}} & \textbf{Average} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-14}
&$R@1$ &$R@2$ &$R@3$ &$R@1$ &$R@2$ &$R@3$ &$R@1$ &$R@2$ &$R@3$ &$R@1$ &$R@2$ &$R@3$ & $R@1$ \\
\midrule
Pic2Word &15.65 &28.16 &38.65 &13.87 &24.67 &33.05 &8.42 &18.01 &25.77 &6.68 &15.05 &24.03 &11.15 \\
SEARLE &17.10 &29.60 &40.70 &\textbf{16.30} &25.20 &34.20 &12.00 &22.20 &30.90 &12.00 &24.10 &33.90 &14.35 \\
LinCIR &16.90 &29.95 &41.45 &16.19 &27.98 &36.84 &8.27 &17.40 &26.22 &7.40 &15.71 &25.00 &12.19\\
CIReVL &19.50 &31.80 &42.00 &14.40 &26.00 &35.20 &12.30 &21.80 &30.50 &\textbf{17.20} &28.90 &37.60 &15.85 \\
\midrule
\textbf{InstructCIR} &\textbf{21.25} &\textbf{34.55} &\textbf{46.85} &16.15 &\textbf{28.74} &\textbf{39.73} &\textbf{17.55} &\textbf{28.01} &\textbf{36.94} &17.04 &\textbf{28.98} &\textbf{37.70} &\textbf{18.00} \\
\bottomrule
\end{tabular}
\caption{\textbf{Comparison of Zero-Shot CIR Models on GeneCIS}.}
\label{tab: complete_genecis_results}
\end{table*}

\begin{table}[ht]
\centering
\begin{tabular}{c|c}
\hline
% \toprule
\textbf{Training Config} & \textbf{Value} \\ \hline
DeepSpeed & ZeRO-2 \\ 
LoRA R & 64 \\
LoRA Alpha & 16 \\
Model Max Length & 512 \\
Precision & FP16 \\
Epochs for both stages & 1 \\
Batch Size Per GPU in Stage 1 & 48 \\
Batch Size Per GPU in Stage 2 & 64 \\
Gradient Accumulation Steps & 1 \\
Learning Rate & 2E-05 \\
Weight Decay & 0 \\
Warm Up Ratio & 0.03 \\
LR Scheduler Type & Cosine \\ \hline
\end{tabular}
\caption{Configurations of Training InstructCIR.}
\label{tab: icir_config}
\end{table}

\section{Training Details}
\label{sec: train_details}
\subsection{MLLM Training}
We use the code and data from xtuner/llava-phi-3-mini-hf~\citep{2023xtuner} to train a variant of LLaVA-Phi. \textit{Note that the goal of this step is solely to make our experiments consistent with the baselines.} Section 4.3 has demonstrated that our training strategy can be directly applied to existing MLLMs. The checkpoint of the variant LLaVA-Phi will also be released for reproducibility. MLLM training and model details are provided in Table \ref{tab: mllm_config}. In addition, InstructCIR and InstructCIR+ leverage on-device MLLMs which are much smaller than the current work E5-V~\cite{jiang2024e5}. Their numbers of parameters are shown in Table \ref{tab: model_size}.

\subsection{InstructCIR Training}
Detailed training configs are shown in Table \ref{tab: icir_config}.

\section{More Experiment Results}
\label{sec: more_results}

Table \ref{tab: complete_genecis_results} shows the complete results on GeneCIS.

% \begin{table*}[ht]
% \scriptsize
% \centering
% \begin{tabular}{lcccccccccccc}
% \toprule
%    & \multirow{3}{*}{Method} & \multicolumn{6}{c}{\textbf{CIRR}} & \multicolumn{4}{c}{\textbf{CIRCO}} \\ 
% \cmidrule(lr){3-8} \cmidrule(lr){9-12}
%    &      & R@1   & R@5   & R@10 & R_s @1 & R_s @2 & R_s @3 & mAP@5 & mAP@10 & mAP@25 & mAP@50 \\
% \midrule
% & InstructCIR_{lp} & 35.08 & \textbf{65.25} & 76.53 & 67.52 & 84.13 & 92.08 & 22.19 & 23.62 & 26.01 & 27.20 \\
% & InstructCIR_{full} & \textbf{35.18} & 65.12 & \textbf{77.61} & \textbf{67.54} & \textbf{84.77} & \textbf{93.61} & \textbf{22.32} & \textbf{23.80}   & \textbf{26.25}  & \textbf{27.32} \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{Comparison of Zero-Shot CIR Models on CIRCO and CIRR Test Sets.} InstructCIR$_{lp}$ refers to InstructCIR that is trained with LLaVA-Pretrain only in the first training stage. InstructCIR$_{full}$ is trained with both LLaVA-Pretrain and FOIL in the first training stage.}
% \label{tab:cirr_and_circo_lp}
% \end{table*}

% \begin{table*}[!h]
% \scriptsize
% \centering
% \begin{tabular}{lccccccc|cccc}
% \toprule
%  & \multirow{3}{*}{Method} & \multicolumn{2}{c}{\textbf{Shirt}} & \multicolumn{2}{c}{\textbf{Dress}} & \multicolumn{2}{c}{\textbf{Toptee}} & \multicolumn{2}{c}{\textbf{Average}} \\ 
% \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
%  & & R@10 & R@50 & R@10 & R@50 & R@10 & R@50 & R@10 & R@50 \\ 
% \midrule
% & InstructCIR_{lp} & 29.85 & 49.98 & 25.04 & 45.60 & 31.74 & 53.26 & 28.90 & 49.61\\
% & InstructCIR_{full} & \textbf{30.96} & \textbf{50.10} & \textbf{25.11} & \textbf{46.18} & \textbf{32.32} & \textbf{54.22} & \textbf{29.46} & \textbf{50.16} \\ 
% % \midrule
% % \multirow{5}{*}{\textbf{ViT-G}} 
% % & Pic2word & 33.17 & 50.39 & 25.43 & 47.65 & 35.24 & 57.62 & 31.28 & 51.89 \\ 
% % & SEARLE & 36.46 & 55.35 & 28.16 & 50.32 & 39.83 & 61.45 & 34.81 & 55.71 \\ 
% % & CIReVL & 33.71 & 51.42 & 27.07 & 49.53 & 35.8 & 56.14 & 32.19 & 52.36 \\ 
% % & LinCIR & 46.76 & 65.11 & 38.08 & 60.88 & 50.48 & 71.09 & 45.11 & 65.69 \\ 
% % \midrule
% % & Ours & - & - & - & - & - & - & - & - \\ 
% \bottomrule
% \end{tabular}%
% % \caption{\textbf{Comparison on FashionIQ}. Ours is able to significantly outperform state-of-the-art methods across all Fashion-IQ sub-benchmarks}
% \caption{\textbf{Comparison of Zero-Shot CIR Models on FashionIQ}. InstructCIR$_{lp}$ refers to InstructCIR that is trained with LLaVA-Pretrain only in the first training stage. InstructCIR$_{full}$ is trained with both LLaVA-Pretrain and FOIL in the first training stage.}
% \label{tab: fiq_results_lp}
% \end{table*}
% \begin{table*}[!h]
% \centering
% \setlength{\tabcolsep}{5pt}
% \scriptsize
% \begin{tabular}{cccccccccccccc}\toprule
% \multirow{2}{*}{\multirow{2}{*}{Method}} &\multicolumn{3}{c}{\textbf{Focus Attribute}} &\multicolumn{3}{c}{\textbf{Change Attribute}} &\multicolumn{3}{c}{\textbf{Focus Object}} &\multicolumn{3}{c}{\textbf{Change Object}} & \textbf{Average} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-14}
% &R@1 &R@2 &R@3 &R@1 &R@2 &R@3 &R@1 &R@2 &R@3 &R@1 &R@2 &R@3 & R@1 \\
% \midrule
% InstructCIR_{lp} & 20.35 & 33.35 & 45.05 & 15.39 & 28.39 & 37.69 & 16.58 & 26.69 & \textbf{37.19} & \textbf{17.14} & 27.86 & \textbf{38.62} & 17.37 \\
% InstructCIR_{full}&\textbf{21.25} &\textbf{34.55} &\textbf{46.85} &\textbf{16.15} &\textbf{28.74} &\textbf{39.73} &\textbf{17.55} &\textbf{28.01} & 36.94 &17.04 &\textbf{28.98} &37.70 &\textbf{18.00} \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{Comparison of Zero-Shot CIR Models on GeneCIS}. InstructCIR$_{lp}$ refers to InstructCIR that is trained with LLaVA-Pretrain only in the first training stage. InstructCIR$_{full}$ is trained with both LLaVA-Pretrain and FOIL in the first training stage.}
% \label{tab: genecis_results_lp}
% \end{table*}

\begin{figure*}
    \centering
    \includegraphics[width=0.7\linewidth]{images/vis_example.pdf}
    \caption{Triplet Examples from CC3M-Instruct}
    \label{fig: vis_example}
\end{figure*}
